Codec-SUPERB: An In-Depth Analysis of Sound Codec Models

The sound codec's dual roles in minimizing data transmission latency and serving as tokenizers underscore its critical importance. Recent years have witnessed significant developments in codec models. The ideal sound codec should preserve content, paralinguistics, speakers, and audio information. However, the question of which codec achieves optimal sound information preservation remains unanswered, as in different papers, models are evaluated on their selected experimental settings. This study introduces Codec-SUPERB, an acronym for Codec sound processing Universal PERformance Benchmark. It is an ecosystem designed to assess codec models across representative sound applications and signal-level metrics rooted in sound domain knowledge.Codec-SUPERB simplifies result sharing through an online leaderboard, promoting collaboration within a community-driven benchmark database, thereby stimulating new development cycles for codecs. Furthermore, we undertake an in-depth analysis to offer insights into codec models from both application and signal perspectives, diverging from previous codec papers mainly concentrating on signal-level comparisons. Finally, we will release codes, the leaderboard, and data to accelerate progress within the community.

==> 0._figures_latex/signal_all_metrics_audio.tex <==
\begin{figure*}[h]
\label{signal_all_metrics_audio}
\centering
\begin{tabular}{cccc}
    \includegraphics[width=0.24\linewidth]{figures/ESC-50/ESC-50 Mel Distance vs kbps.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/FSD-50K/FSD50K Mel Distance vs kbps.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/Gunshot Triangulation/Gunshot Triangulation Mel Distance vs kbps.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/Vocal Imitations/Vocal Imitations Mel Distance vs kbps.pdf}\\
    \includegraphics[width=0.24\linewidth]{figures/ESC-50/ESC-50 STFT Distance vs kbps.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/FSD-50K/FSD50K STFT Distance vs kbps.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/Gunshot Triangulation/Gunshot Triangulation STFT Distance vs kbps.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/Vocal Imitations/Vocal Imitations STFT Distance vs kbps.pdf}\\

    (a) ESC-50 & (b) VoxCeleb1 & (c) Speech Commands v1 & (d) QUESST \\    
\end{tabular}
\caption{Objective metrics for 4 audio dataset}
\end{figure*}
% \begin{figure*}[h]
% \label{signal_all_metrics_audio}
% \centering
% \begin{tabular}{cccc}
%     \includegraphics[width=0.24\linewidth]{figures/ESC-50/mel.png}&
%     \includegraphics[width=0.24\linewidth]{figures/FSD-50K/mel.png}&
%     \includegraphics[width=0.24\linewidth]{figures/Gunshot Triangulation/mel.png}&
%     \includegraphics[width=0.24\linewidth]{figures/Vocal Imitations/mel.png}\\
%     \includegraphics[width=0.24\linewidth]{figures/ESC-50/stft.png}&
%     \includegraphics[width=0.24\linewidth]{figures/FSD-50K/stft.png}&
%     \includegraphics[width=0.24\linewidth]{figures/Gunshot Triangulation/stft.png}&
%     \includegraphics[width=0.24\linewidth]{figures/Vocal Imitations/stft.png}\\
%     % \includegraphics[width=0.24\linewidth]{figures/ESC-50/pesq.png}&
%     % \includegraphics[width=0.24\linewidth]{figures/FSD-50K/pesq.png}&
%     % \includegraphics[width=0.24\linewidth]{figures/Gunshot Triangulation/pesq.png}&
%     % \includegraphics[width=0.24\linewidth]{figures/Vocal Imitations/pesq.png}\\
%     (a) ESC-50 & (b) VoxCeleb1 & (c) Speech Commands v1 & (d) QUESST \\    
% \end{tabular}
% \caption{Objective metrics for 4 audio dataset}
% \end{figure*}

==> 0._figures_latex/signal_all_metrics_music_2.tex <==
\begin{figure*}[h]
\label{signal_all_metrics_music_2}
\centering
\begin{tabular}{cc}
    \includegraphics[width=0.24\linewidth]{figures/GTZAN Genre/mel.png}&
    \includegraphics[width=0.24\linewidth]{figures/GTZAN Music Speech/mel.png}\\
    \includegraphics[width=0.24\linewidth]{figures/GTZAN Genre/stft.png}&
    \includegraphics[width=0.24\linewidth]{figures/GTZAN Music Speech/stft.png}\\
    \includegraphics[width=0.24\linewidth]{figures/GTZAN Genre/pesq.png}&
    \includegraphics[width=0.24\linewidth]{figures/GTZAN Music Speech/pesq.png}\\
    \includegraphics[width=0.24\linewidth]{figures/GTZAN Genre/stoi.png}&
    \includegraphics[width=0.24\linewidth]{figures/GTZAN Music Speech/stoi.png}\\
    % \includegraphics[width=0.24\linewidth]{figures/GTZAN Genre/f0corr.png}&
    % \includegraphics[width=0.24\linewidth]{figures/GTZAN Music Speech/f0corr.png}\\
    (e) GTZAN Genre & (f) GTZAN Music Speech \\
\end{tabular}
\caption{Objective metrics for 2 music dataset}
\end{figure*}

==> 0._figures_latex/signal_all_metrics_music_4.tex <==
\begin{figure*}[h]
\label{signal_all_metrics_music_4}
\centering
\begin{tabular}{cccc}
    \includegraphics[width=0.24\linewidth]{figures/OpenSinger/mel.png}&
    \includegraphics[width=0.24\linewidth]{figures/M4Singer/mel.png}&
    \includegraphics[width=0.24\linewidth]{figures/VocalSet/mel.png}&
    \includegraphics[width=0.24\linewidth]{figures/NSynth/mel.png}\\
    \includegraphics[width=0.24\linewidth]{figures/OpenSinger/stft.png}&
    \includegraphics[width=0.24\linewidth]{figures/M4Singer/stft.png}&
    \includegraphics[width=0.24\linewidth]{figures/VocalSet/stft.png}&
    \includegraphics[width=0.24\linewidth]{figures/NSynth/stft.png}\\
    \includegraphics[width=0.24\linewidth]{figures/OpenSinger/pesq.png}&
    \includegraphics[width=0.24\linewidth]{figures/M4Singer/pesq.png}&
    \includegraphics[width=0.24\linewidth]{figures/VocalSet/pesq.png}&
    \includegraphics[width=0.24\linewidth]{figures/NSynth/pesq.png}\\
    \includegraphics[width=0.24\linewidth]{figures/OpenSinger/stoi.png}&
    \includegraphics[width=0.24\linewidth]{figures/M4Singer/stoi.png}&
    \includegraphics[width=0.24\linewidth]{figures/VocalSet/stoi.png}&
    \includegraphics[width=0.24\linewidth]{figures/NSynth/stoi.png}\\
    \includegraphics[width=0.24\linewidth]{figures/OpenSinger/f0corr.png}&
    \includegraphics[width=0.24\linewidth]{figures/M4Singer/f0corr.png}&
    \includegraphics[width=0.24\linewidth]{figures/VocalSet/f0corr.png}&
    \includegraphics[width=0.24\linewidth]{figures/NSynth/f0corr.png}\\
    (a) OpenSinger & (b) M4Singer & (c) VocalSet & (d) NSynth \\
\end{tabular}
\caption{Objective metrics for 4 music dataset}
\end{figure*}

==> 0._figures_latex/signal_all_metrics_speech_2.tex <==
\begin{figure*}[h]
\label{signal_all_metrics_speech_2}
\centering
\begin{tabular}{cccc}
    \includegraphics[width=0.24\linewidth]{figures/Libri2Mix/mel.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/LibriCount/mel.pdf}\\
    \includegraphics[width=0.24\linewidth]{figures/Libri2Mix/stft.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/LibriCount/stft.pdf}\\
    \includegraphics[width=0.24\linewidth]{figures/Libri2Mix/pesq.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/LibriCount/pesq.pdf}\\
    \includegraphics[width=0.24\linewidth]{figures/Libri2Mix/stoi.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/LibriCount/stoi.pdf}\\
    (i) Libri2Mix & (j) LibriCount \\
\end{tabular}
\caption{Objective metrics for 2 speech dataset}
\end{figure*}

==> 0._figures_latex/signal_all_metrics_speech_8.tex <==
\begin{figure*}[h]
\label{signal_all_metrics_speech_8}
\centering
\begin{tabular}{cccc}
    \includegraphics[width=0.24\linewidth]{figures/Librispeech/mel.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/VoxCeleb1/mel.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/Speech Commands v1/mel.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/QUESST/mel.pdf}\\
    \includegraphics[width=0.24\linewidth]{figures/Librispeech/stft.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/VoxCeleb1/stft.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/Speech Commands v1/stft.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/QUESST/stft.pdf}\\
    \includegraphics[width=0.24\linewidth]{figures/Librispeech/pesq.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/VoxCeleb1/pesq.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/Speech Commands v1/pesq.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/QUESST/pesq.pdf}\\
    \includegraphics[width=0.24\linewidth]{figures/Librispeech/stoi.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/VoxCeleb1/stoi.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/Speech Commands v1/stoi.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/QUESST/stoi.pdf}\\
    (a) Librispeech & (b) VoxCeleb1 & (c) Speech Commands v1 & (d) QUESST \\
    \includegraphics[width=0.24\linewidth]{figures/VoxLingua107 Top 10/mel.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/Audio SNIPS/mel.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/IEMOCAP/mel.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/CREMA-D/mel.pdf}\\
    \includegraphics[width=0.24\linewidth]{figures/VoxLingua107 Top 10/stft.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/Audio SNIPS/stft.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/IEMOCAP/stft.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/CREMA-D/stft.pdf}\\
    \includegraphics[width=0.24\linewidth]{figures/VoxLingua107 Top 10/pesq.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/Audio SNIPS/pesq.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/IEMOCAP/pesq.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/CREMA-D/pesq.pdf}\\
    \includegraphics[width=0.24\linewidth]{figures/VoxLingua107 Top 10/stoi.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/Audio SNIPS/stoi.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/IEMOCAP/stoi.pdf}&
    \includegraphics[width=0.24\linewidth]{figures/CREMA-D/stoi.pdf}\\
    (e) VoxLingua107 Top 10 & (f) Audio SNIPS & (g) IEMOCAP & (h) CREMA-D \\
    
\end{tabular}
\caption{Objective metrics for 8 speech dataset}
\end{figure*}

==> 0._tables_latex/audio_snips.tex <==
% Eric
\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccc}
\toprule
\textbf{Codec} & \textbf{{MelDistance $\downarrow$}} & \textbf{{STFTDistance $\downarrow$}} & \textbf{{PESQ $\uparrow$}} & \textbf{{STOI $\uparrow$}} & \textbf{{Overall Score $\uparrow$}} \\
\midrule
A & 0.890 & 2.087 & 2.416 & 0.927 & 0.697 \\
\midrule
B1 & 1.797 & 3.282 & 2.564 & 0.939 & 0.666 \\
B2 & 1.738 & 3.312 & 2.397 & 0.925 & 0.655 \\
B3 & 1.761 & 3.194 & 2.469 & 0.940 & 0.662 \\
\midrule
C & 1.097 & 2.248 & 1.978 & 0.832 & 0.639 \\
\midrule
D1 & 0.624 & 1.688 & 3.766 & 0.977 & 0.808 \\
D2 & 0.375 & 1.433 & 4.335 & 0.995 & 0.868 \\
D3 & 0.687 & 1.829 & 3.669 & 0.974 & 0.794 \\
\midrule
E1 & 1.254 & 2.439 & 1.554 & 0.861 & 0.596 \\
E2 & 1.074 & 2.234 & 2.045 & 0.912 & 0.656 \\
E3 & 0.935 & 2.085 & 2.687 & 0.948 & 0.716 \\
E4 & 0.813 & 1.963 & 3.304 & 0.971 & 0.764 \\
E5 & 0.749 & 1.903 & 3.643 & 0.980 & 0.787 \\
\midrule
F1 & 0.823 & 1.789 & 3.477 & 0.901 & 0.764 \\
F2 & 0.764 & 1.701 & 3.479 & 0.906 & 0.771 \\
F3 & 0.743 & 1.723 & 3.308 & 0.974 & 0.775 \\
F4 & 0.797 & 1.779 & 3.013 & 0.966 & 0.753 \\
F5 & 0.703 & 1.677 & 3.562 & 0.979 & 0.793 \\
F6 & 0.751 & 1.767 & 3.221 & 0.973 & 0.769 \\
\bottomrule
\end{tabular}
}
\caption{Signal-level metrics for Audio SNIPS}
\label{tab:metric_Audio SNIPS}
\end{table}

==> 0._tables_latex/downstream_overall_performance.tex <==
% \begin{table}[t]
% \centering
% \caption{Downstream task performance. ``None'' means that no codec has been applied.}
% \label{tab:downstream_performance}
% \begin{tabular}{lccccc}
% \toprule
% \textbf{Codec} & \textbf{WER (ASR) $\downarrow$} & \textbf{EER (ASV) $\downarrow$} & \textbf{minDCF (ASV) $\downarrow$} & \textbf{ACC (ER) $\uparrow$} & \textbf{mAP (AEC) $\uparrow$} \\
% \toprule
% None & 2.96\% & 0.86\% & 0.07\% & 69.84\% & 45.68\% \\
% \midrule
% A & 4.02\% & 3.31\% & 0.24\% & 65.49\%  &  15.11\%  \\
% \midrule
% B1 & 4.94\% & 4.43\% & 0.29\% & 65.96\% &  16.19\%  \\
% B2 & 6.26\% & 5.22\% & 0.38\% & 64.63\% &  28.65\%  \\
% B3 & 4.49\% & 6.16\% & 0.36\% & 65.95\% &  14.01\%  \\
% \midrule
% C & 3.94\% & 5.22\% & 0.30\% & 65.70\%  &  17.41\%  \\
% \midrule
% D1 & 3.26\% & 1.59\% & 0.12\% & 68.81\% &  41.08\%  \\
% D2 & 2.96\% & 2.24\% & 0.14\% & 69.56\% &  41.37\%  \\
% D3 & 3.18\% & 3.59\% & 0.26\% & 69.18\% &  32.04\%  \\
% \midrule
% E1 & 9.21\% & 13.88\% & 0.68\% & 58.84\% &  18.84\% \\
% E2 & 4.34\% & 6.85\% & 0.39\% & 63.54\%  &  26.63\% \\
% E3 & 3.49\% & 4.28\% & 0.27\% & 66.18\% &  32.43\% \\
% E4 & 3.22\% & 3.44\% & 0.21\% & 67.63\% &  35.84\% \\
% E5 & 3.17\% & 3.15\% & 0.19\% & 68.26\% &  36.64\% \\
% \midrule
% F1 & 3.21\% & 1.50\% & 0.10\% & 63.54\% & 37.31\%    \\
% F2 & 3.16\% & 1.81\% & 0.10\% & 66.18\% & 37.77\%    \\
% F3 & 3.28\% & 1.76\% & 0.12\% & 67.63\% & 25.52\%    \\
% F4 & 3.43\% & 2.04\% & 0.13\% & 68.26\% & 21.43\%    \\
% F5 & 3.21\% & 1.52\% & 0.11\% & 69.25\% & 26.42\%    \\
% F6 & 3.27\% & 1.60\% & 0.11\% & 69.55\% & 33.59\%    \\
% \bottomrule
% \end{tabular}
% \end{table}

%%%%%%%%%%% resize by Xuanjun in 2024.02.14 1:43 PM %%%%%%%%%%%%
\begin{table}[t]\scriptsize
\resizebox{0.48\textwidth}{!}{%
\begin{minipage}{0.45\textwidth}
\centering
\begin{tabular}{lccccc}
\toprule
% \textbf{Codec} & \textbf{WER (ASR) $\downarrow$} & \textbf{EER (ASV) $\downarrow$} & \textbf{minDCF (ASV) $\downarrow$} & \textbf{ACC (ER) $\uparrow$} & \textbf{mAP (AEC) $\uparrow$} \\
\textbf{Codec} & \textbf{WER$\downarrow$} & \textbf{EER$\downarrow$} & \textbf{minDCF$\downarrow$} & \textbf{ACC$\uparrow$} & \textbf{mAP $\uparrow$} \\
 & \textbf{(ASR)} & \textbf{(ASV)} & \textbf{(ASV)} & \textbf{(ER)} & \textbf{(AEC)} \\
\toprule
None & 2.96\% & 0.86\% & 0.07\% & 69.84\% & 45.68\% \\
\midrule
A & 4.02\% & 3.31\% & 0.24\% & 65.49\%  &  15.11\%  \\
\midrule
B1 & 4.94\% & 4.43\% & 0.29\% & 65.96\% &  16.19\%  \\
B2 & 6.26\% & 5.22\% & 0.38\% & 64.63\% &  28.65\%  \\
B3 & 4.49\% & 6.16\% & 0.36\% & 65.95\% &  14.01\%  \\
\midrule
C & 3.94\% & 5.22\% & 0.30\% & 65.70\%  &  17.41\%  \\
\midrule
D1 & 3.26\% & 1.59\% & 0.12\% & 68.81\% &  41.08\%  \\
D2 & 2.96\% & 2.24\% & 0.14\% & 69.56\% &  41.37\%  \\
D3 & 3.18\% & 3.59\% & 0.26\% & 69.18\% &  32.04\%  \\
\midrule
E1 & 9.21\% & 13.88\% & 0.68\% & 58.84\% &  18.84\% \\
E2 & 4.34\% & 6.85\% & 0.39\% & 63.54\%  &  26.63\% \\
E3 & 3.49\% & 4.28\% & 0.27\% & 66.18\% &  32.43\% \\
E4 & 3.22\% & 3.44\% & 0.21\% & 67.63\% &  35.84\% \\
E5 & 3.17\% & 3.15\% & 0.19\% & 68.26\% &  36.64\% \\
\midrule
F1 & 3.21\% & 1.50\% & 0.10\% & 63.54\% & 37.31\%    \\
F2 & 3.16\% & 1.81\% & 0.10\% & 66.18\% & 37.77\%    \\
F3 & 3.28\% & 1.76\% & 0.12\% & 67.63\% & 25.52\%    \\
F4 & 3.43\% & 2.04\% & 0.13\% & 68.26\% & 21.43\%    \\
F5 & 3.21\% & 1.52\% & 0.11\% & 69.25\% & 26.42\%    \\
F6 & 3.27\% & 1.60\% & 0.11\% & 69.55\% & 33.59\%    \\
\bottomrule
\end{tabular}
\caption{Downstream task performance. ``None'' means that no codec has been applied.}
\label{tab:downstream_performance}
\end{minipage}
}%
\end{table}

% \begin{table}[t]
% \resizebox{0.5\textwidth}{!}{%
% \begin{minipage}{\textwidth}
% \centering
% \caption{Downstream task performance. ``None'' means that no codec has been applied.}
% \label{tab:downstream_performance}
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Codec} & \textbf{WER (ASR) $\downarrow$} & \textbf{EER (ASV) $\downarrow$} & \textbf{ACC (ER) $\uparrow$} & \textbf{mAP (AEC) $\uparrow$} \\
% \toprule
% None & 2.96\% & 0.86\% & 69.84\% & 45.68\% \\
% \midrule
% A & 4.02\% & 3.31\% & 65.49\%  &  15.11\%  \\
% \midrule
% B1 & 4.94\% & 4.43\% & 65.96\% &  16.19\%  \\
% B2 & 6.26\% & 5.22\% & 64.63\% &  28.65\%  \\
% B3 & 4.49\% & 6.16\% & 65.95\% &  14.01\%  \\
% \midrule
% C & 3.94\% & 5.22\% & 65.70\%  &  17.41\%  \\
% \midrule
% D1 & 3.26\% & 1.59\% & 68.81\% &  41.08\%  \\
% D2 & 2.96\% & 2.24\% & 69.56\% &  41.37\%  \\
% D3 & 3.18\% & 3.59\% & 69.18\% &  32.04\%  \\
% \midrule
% E1 & 9.21\% & 13.88\% & 58.84\% &  18.84\% \\
% E2 & 4.34\% & 6.85\% & 63.54\%  &  26.63\% \\
% E3 & 3.49\% & 4.28\% & 66.18\% &  32.43\% \\
% E4 & 3.22\% & 3.44\% & 67.63\% &  35.84\% \\
% E5 & 3.17\% & 3.15\% & 68.26\% &  36.64\% \\
% \midrule
% F1 & 3.21\% & 1.50\% & 63.54\% & 37.31\%    \\
% F2 & 3.16\% & 1.81\% & 66.18\% & 37.77\%    \\
% F3 & 3.28\% & 1.76\% & 67.63\% & 25.52\%    \\
% F4 & 3.43\% & 2.04\% & 68.26\% & 21.43\%    \\
% F5 & 3.21\% & 1.52\% & 69.25\% & 26.42\%    \\
% F6 & 3.27\% & 1.60\% & 69.55\% & 33.59\%    \\
% \bottomrule
% \end{tabular}
% \end{minipage}
% }%
% \end{table}

==> 0._tables_latex/signal_level_overall_performance.tex <==
\begin{table}[t]\scriptsize
\resizebox{0.48\textwidth}{!}{%
\begin{minipage}{0.45\textwidth}
\centering
\begin{tabular}{lccc}
\toprule
\textbf{Codec} & \textbf{Speech Overall $\uparrow$} & \textbf{Audio Overall $\uparrow$} & \textbf{Music Overall $\uparrow$} \\
% \textbf{Codec} & \textbf{Speech $\uparrow$} & \textbf{Audio $\uparrow$} & \textbf{Music $\uparrow$} \\
\toprule
A & 0.644 & 0.581 & 0.585 \\
\midrule
B1 & 0.610 & 0.574 & 0.601 \\
B2 & 0.617 & 0.574 & 0.630 \\
B3 & 0.611 & 0.592 & 0.604 \\
\midrule
C & 0.596 & 0.602 & 0.572 \\
\midrule
D1 & 0.798 & 0.591 & 0.749 \\
D2 & 0.864 & 0.636 & 0.815 \\
D3 & 0.802 & 0.702 & 0.770 \\
\midrule
E1 & 0.579 & 0.594 & 0.568 \\
E2 & 0.636 & 0.599 & 0.621 \\
E3 & 0.697 & 0.602 & 0.669 \\
E4 & 0.748 & 0.606 & 0.710 \\
E5 & 0.775 & 0.609 & 0.732 \\
\midrule
F1 & 0.724 & 0.582 & 0.667 \\
F2 & 0.704 & 0.583 & 0.668 \\
F3 & 0.705 & 0.581 & 0.649 \\
F4 & 0.678 & 0.578 & 0.632 \\
F5 & 0.726 & 0.583 & 0.665 \\
F6 & 0.718 & 0.583 & 0.667 \\
\bottomrule
\end{tabular}
\caption{Signal-level overall score}
\label{tab:signal_level_overall_scores}
\end{minipage}
}%
\end{table}

==> 0._tables_latex/table_codec_information.tex <==
%%%%%%%%%%% resize by Xuanjun in 2024.02.14 1:43 PM %%%%%%%%%%%%
% \begin{table}[htbp]
\begin{table}[t]
\centering
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{lccc}
\toprule
\textbf{Codec name} & \textbf{Mark} & \textbf{SR} & \textbf{kbps} \\
\midrule
speech\_tokenizer\_16k & A & 16 & 4 \\
\midrule
academicodec\_hifi\_16k\_320d & B1 & 16 & 2 \\
academicodec\_hifi\_16k\_320d\_large\_uni & B2 & 16 & 2 \\
academicodec\_hifi\_24k\_320d & B3 & 24 & 3 \\
\midrule
audiodec\_24k\_320d & C & 24 & 6.4 \\
\midrule
dac\_16k & D1 & 16 & 6 \\
dac\_24k & D2 & 24 & 24 \\
dac\_44k & D3 & 44.1 & 8 \\
\midrule
encodec\_24k\_1.5kbps & E1 & 24 & 1.5 \\
encodec\_24k\_3kbps & E2 & 24 & 3 \\
encodec\_24k\_6kbps & E3 & 24 & 6 \\
encodec\_24k\_12kbps & E4 & 24 & 12 \\
encodec\_24k\_24kbps & E5 & 24 & 24 \\
\midrule
funcodec\_en\_libritts\_16k\_gr1nq32ds320 & F1 & 16 & 16 \\
funcodec\_en\_libritts\_16k\_gr8nq32ds320 & F2 & 16 & 16 \\
funcodec\_en\_libritts\_16k\_nq32ds320 & F3 & 16 & 16 \\
funcodec\_en\_libritts\_16k\_nq32ds640 & F4 & 16 & 8 \\
funcodec\_zh\_en\_16k\_nq32ds320 & F5 & 16 & 16 \\
funcodec\_zh\_en\_16k\_nq32ds640 & F6 & 16 & 8 \\
\bottomrule
\end{tabular}
}%
\caption{Codec information. Sample rate (SR) is in kHz.}
\label{tab:codec_info}
\end{table}

